Understanding How Dimension Reduction Tools Work: An Empirical Approach to Deciphering t-SNE, UMAP, TriMAP, and PaCMAP for Data Visualization

Dimension reduction (DR) techniques such as t-SNE, UMAP, and TriMAP have demonstrated impressive visualization performance on many real world datasets. One tension that has always faced these methods is the trade-off between preservation of global structure and preservation of local structure: these methods can either handle one or the other, but not both. In this work, our main goal is to understand what aspects of DR methods are important for preserving both local and global structure: it is difficult to design a better method without a true understanding of the choices we make in our algorithms and their empirical impact on the lower-dimensional embeddings they produce. Towards the goal of local structure preservation, we provide several useful design principles for DR loss functions based on our new understanding of the mechanisms behind successful DR methods. Towards the goal of global structure preservation, our analysis illuminates that the choice of which components to preserve is important. We leverage these insights to design a new algorithm for DR, called Pairwise Controlled Manifold Approximation Projection (PaCMAP), which preserves both local and global structure. Our work provides several unexpected insights into what design choices both to make and avoid when constructing DR algorithms.

==> ToDo.tex <==
DO NOT EDIT THIS ONE!




formalize pacmap (Yingfan) (use notation)
include drafts of all figures in overleaf (for each figure, keep track of the hyper-parameters used to generate it) (Haiyang)
create the bad loss function plots (see fake loss functions in google doc)(Yingfan) + TSNE loss plot
ask Ed about data (Cynthia)
read sec 4 (Cynthia and Yaron)
fix figures 1 and 2 (Haiyang)


To do: 1) Someone try to figure out equation 1 and whether it is the objective in UMAP
To do 2) Yaron: section 4.1 and 4.2 outline
To do 3) Cynthia talk with Ed on the bio data
Section 4.3 on initialization
Section 4.4: list all the experiments relating to the optimization 
to do 6: start filling section 6 on the numerical experiments
Everyone should read sec 5 formal definition of pacmap

Meeting 2020/05/21
------------------
1) Add footnote, about discrepancy between the paper and the implementation
2) start section 4 with high-level description of the loss as summation of graph components $\sum _{components} loss(componenets_H, componenets_L)$
3) add to section 4 list of alternative loss functions that we tried
4) (explain better the rainbow plots and how they correspond to the elements of a good loss function) add note: rainbow figure - shows simultaneously the gradient for the near and far 
5) consider adding a plot similar to t-sne paper page 8, gradient as a function of high and low dimensional distances




Meeting 2020/08/05
1) consider a metric to measure local structure preservation which is how many high dim neighbors do we preserve in low dim

Yaron
- try alternative losses that fit our priniciples, e.g., like unimodal probability distribution
- expand numerical experiments with other algorithms and datasets
- appendix B illustrates how we can test if a graph layout algorithm is appropriate for DR. Potentially, we could choose the top 5-10 methods, apply DR and show that there is a 1-1 (hopefully) mapping between DR methods that work and our principles
- 
- 
- 


==> coverletter.tex <==
September 24, 2020

Dear JMLR Editors, 
We are pleased to submit our manuscript, “Understanding How Dimension Reduction Tools Work: An Empirical Approach to Deciphering t-SNE, UMAP, TriMAP, and PaCMAP for Data Visualization” for possible publication in the Journal of Machine Learning Research.
Our work provides new insights into what aspects of dimension reduction (DR) methods are important for preserving both local and global structure: it is difficult to design a better method without a true understanding of the choices we make in our algorithms and their empirical impact on the lower-dimensional embeddings they produce. Towards the goal of local structure preservation, we provide several useful design principles for DR loss functions based on our new understanding of the mechanisms behind successful DR methods. Towards the goal of global structure preservation, our analysis illuminates that the choice of which components to preserve is important. We leverage these insights to design a new algorithm for DR, called Pairwise Controlled Manifold Approximation Projection (PaCMAP), which preserves both local and global structure. Our work provides several unexpected insights into what design choices both to make and avoid when constructing DR algorithms.
This manuscript is not under review elsewhere and all authors approve of its submission to JMLR. We believe that this manuscript would be an excellent fit for the journal which published highly impactful papers in this area, and which our work relates to. Finally, we have no conflicts of interest to disclose. 
Suggested AE’s: We suggest that the AE have an appreciation for applied work. It doesn’t seem that JMLR has many AE’s whose central research area is dimension reduction for data visualization, but someone who works in this area would be ideal. Possibilities of suitable AE’s would be Russ Greiner and Tina Eliassi-Rad who are data miners that work in applied areas.

AE’s that we do not recommend: Moritz Hardt, Corinna Cortes, Edoardo Airoldi, Mehryar Mohri, and Joris Mooij.
Thank you for your consideration and we look forward to your review.
Sincerely,
Yingfan Wang, Haiyang Huang, Cynthia Rudin, and Yaron Shaposhnik. 


